IXPE observations of supernova remnants

Supernova remnants (SNRs) are among the most important sources of non-thermal X-rays in the sky and likely contributors to Galactic cosmic rays and represent ideal targets to showcase the capabilities of the Imaging X-ray Polarimetry Explorer (IXPE) in performing spatially-resolved X-ray polarimetry. For the first time, we can determine the turbulence level (through the measurement of polarization degree) and the orientation (through polarization direction) of the magnetic field near the shocks, where particle acceleration occurs. IXPE reported so far the results of the observations of four SNRs: Cas A, Tycho, SN 1006 and RX J1713.7-3946. These objects exhibit a wide range of characteristics, including dynamical age, spectral composition of emission, and progenitor type. Aptly, they revealed significantly different results among them in terms of magnetic field properties and morphology, providing unexpected insights and shedding light on the particle acceleration mechanisms in astrophysical shocks.

==> organizers.tex <==
%to switch ON running title
%\markboth{Organizing committees}{Organizing committees}

\wstoc{Organizing committees}{}

\title{Organizing committees}

\begin{center}
{\bf Series editorial board}\\
{\it for the series on advances in quantum many-body theory}
\end{center}
\vspace*{1em}

\begin{tabular}{ll}
R. F. Bishop (Chairman) & -- UMIST, Manchester, UK\\
C. E. Campbell & -- University of Minnesota, USA \\
J. W. Clark & -- Washington University, St.\ Louis, USA \\
S. Fantoni & -- SISSA, Trieste, Italy
\end{tabular}

\vspace*{0.12in}

\noindent
\begin{center}
{\bf International advisory committee}\\
{\it for the Series of International Conferences on}\\
{\it Recent Progress in Many-Body Theories}
\end{center}
\vspace*{1em}

\noindent
\begin{tabular}{ll}
R. F. Bishop (Chairman) & -- UMIST, Manchester, UK\\
S. Fantoni (Secretary) & -- SISSA, Trieste, Italy\\
C. E. Campbell (Treasurer) & -- University of Minnesota, USA\\
H. K\"{u}mmel (Hon.\ President) & -- Ruhr-Universit\"{a}t
Bochum, Germany \\
J. A. Carlson & -- Los Alamos National Laboratory, USA \\
S. A. Chin & -- Texas A \& M University, USA \\
J. W. Clark & -- Washington University, St.~Louis, USA \\
P. Fulde & -- Max-Planck-Institut f\"{u}r Komplexer  \\
& ~~~Systeme, Dresden, Germany\\
A. Kallio & -- University of Oulu, Finland \\
E. Krotscheck & -- Johannes Universit\"{a}t Linz, Austria \\
C. Lhuillier & -- Universit\'{e} Pierre et Marie Curie, Paris\\
A. MacDonald & -- Indiana University, Bloomington, USA \\
E. Manousakis & -- Florida State University, USA \\
D. Neilson & -- University of New South Wales, Sydney, \\
& ~~~Australia \\
M. L. Ristig & -- Universit\"{a}t zu K\"{o}ln, Germany
\end{tabular}


==> preface.tex <==
%to switch ON running title
%\markboth{Preface}{Preface}

\wstoc{Preface}{}

\title{Preface}

The {\it Tenth International Conference on Recent Progress in
Many-Body Theories} (RPMBT-10) was held at the University of
Washington in Seattle, USA during the period 10-15 September, 1999.
The present volume contains the texts of most of the invited talks
delivered at the conference and a selection from among the many poster
presentations.

The general format and style of the conference followed the accepted
and well-developed pattern for the series, focusing on the
development, refinement and important applications of the techniques
of quantum many-body theory.  The intention of the series has always
been to cover in a broad and balanced fashion both the entire spectrum
of theoretical tools developed to tackle the quantum many-body problem
and their major fields of application.  One of the main aims of the
series is to foster the exchange of ideas and techniques among
physicists working in such diverse areas of applications of many-body
techniques as nuclear and subnuclear physics, astrophysics, atomic and
molecular physics, quantum chemistry, complex systems, quantum field
theory, strongly correlated electronic systems, magnetism, quantum
fluids and condensed matter physics.

Quantum many-body theory as a discipline in its own right dates
largely from the 1950's, and is hence in many senses already a
mature subject.  Despite this apparent maturity the field remains
vibrant and active, vigorous and exciting, vital and important.
Indeed, the successes, importance and vitality of the field have
very clearly been recognized by the sharing of the 1998 Nobel Prizes
in both Physics and Chemistry by the many-body theorists Robert
Laughlin, Walter Kohn and John Pople.  It is a source of great
pleasure to all of us who work in quantum many-body theory that
important achievements in our subject have been thus recognized at
the very highest level.  We were also especially delighted that two
of these then most recent Nobel Laureates, Kohn and Laughlin,
accepted invitations to deliver keynote lectures at RPMBT-10...

A major challenge will be to define and explore these important
areas of overlap in such likely arenas as phase transitions and the
related competing effects of quantum versus thermal fluctuations;
spontaneous symmetry breaking; the unifying role of gauge invariance
(and perhaps other symmetries); concepts from complexity theory,
including the role of correlations and fluctuations in complex
systems, and the competition between analysis and synthesis as modes
of understanding many-body systems; entropy and its generation and
flow; and nonlinearity and its appearance and role at the boundary
between microscopic and mesoscopic descriptions of many-body
systems.  One can perhaps begin to glimpse some insights within the
present proceedings into some of these as areas of future forefront
activity in quantum many-body theory. In this case it may well be
that RPMBT-10 and its immediate successors will later be identified
as the first in the series at which the seeds of the new discourse
between quantum many-body/field theory and statistical physics took
root.

In any event, the Local Organizing and Programme Committees deserve
great thanks in creating a well-run and productive meeting, with an
exciting programme of talks and poster presentations. It is a pleasure
to thank all of them for their hard work, especially Aurel Bulgac who,
as Chairman, has led and guided them throughout.

\vspace*{0.35in}

\noindent
R.F. Bishop \hfill Manchester, U.K.\\
{\itshape (Chairman, International Advisory Committee}
\hfill 31 December 1999\\
{\itshape for the Series of International Conferences on}\\
{\itshape Recent Progress in Many-Body Theories)}


==> proc1.tex <==
%\documentclass{ws-procs961x669}
%\begin{document}

\wstoc{For proceedings editors: Combining contributions\\ using
WS-procs961x669 master document in \LaTeX2e}{F. Author}

\title{For proceedings editors:\\ Combining
contributions using WS-procs961x669\\ master document in \LaTeX2e}

\author{First Author}
\index{author}{Author, F.} % or \aindx{Author, F.}

\address{World Scientific Publishing Co, Production Department,\\
5 Toh Tuck Link, Singapore 596224, \\E-mail: wspc@wspc.com.sg}

\begin{abstract}
ws-procs961x669.tex is the master file to input all the papers from
front matter, body and end matter files.
\end{abstract}

\keywords{Master file; \LaTeX; Proceedings; World Scientific Publishing.}

\section{Master File}
You can obtain these files from the following website:\\
\url{http://www.icpress.co.uk/authors/stylefiles.shtml#conference} and \\
\url{http://www.worldscientific.com/page/authors/proceedings-stylefiles}.

\

All the subdocuments are arranged in this master file in the
following sequence:
\begin{verbatim}
\documentclass{ws-procs961x669}

\usepackage{ws-toc,ws-multind}
\makeindex{author}                    %to invoke author index

\begin{document}
\titlepages
\input preface.tex
\cleardoublepage
\include organizers.tex
\blankpage
\mastertoc
%\part{Part Title}{}                  %optional part title
\include{proc1}
\include{proc2}
%\part{Second Part}{}                 %optional part title
\include{proc3}
\blankpage
\printindex{author}{AUTHOR INDEX}     %to print Author Index
\end{document}
\end{verbatim}

\section{Pagination}

Pages i--iv are always the same and are prepared by the publisher.
The pagination of the rest of the front matter depends on the length
of the various sections (preface, organizing committee's text,
contents). Each front matter section should start on an odd
right-hand page. The following is an example of proceedings
pagination:

\begin{romanlist}[(iii)]

\item Front matter:

\begin{tabular}{@{}lll@{}}
page i &--- & half-title page, prepared by publisher\\
page ii &--- & blank page\\
page iii &--- & full-title page, prepared by publisher\\
page iv &--- & copyright page, prepared by publisher\\
pages v--ix &--- & preface text\\
page xi &--- & organizing committees text\\
pages xiii--xx &--- & contents text (TOC)\\
\end{tabular}\\

The first available front matter page is page v.\\

\item Body text:

\begin{tabular}{@{}lll@{}}
odd page &--- & First article, followed by remaining articles\\
\end{tabular}\\

\item Back matter (optional):

\begin{tabular}{@{}lll@{}}
odd page &--- & participants list\\
\end{tabular}\\

Back matter text must start on an odd page.

\end{romanlist}

\noindent{\bf If the organization of the contributors' manuscripts
is different from the above pagination guidelines, please e-mail the
respective desk-editor for advice.}

\begin{table}
\tbl{This table shows how the author names should appear in running head and TOC depending
upon the number of authors contributing that paper.}
{\begin{tabular}{ll} \toprule
No. of Authors & Author Names\\
\colrule
1 & L. Hatcher\\
2 & I. A. Pedrosa \& I. Guedes\\
3 & B. Feng, X. Gong \& X. Wang\\
4 and more & S. R. Choudhury {\it et al.}\\\botrule
\end{tabular}}
\begin{tabnote}
For TOC and Running Heads, the author names should appear in initial and surname format, e.g. LEE HATCHER should be abbreviated as L.~HATCHER.\\
\end{tabnote}
\end{table}

\section{Running Head}

Preparation of the running head is optional.
Each contribution must have \verb|\markboth| at the preamble to set
the running head.

\verb|\markboth{Author's Name on Even Page}{Article Title on Odd Page}|

\section{Master TOC}

Each contribution must have \verb|\wstoc{#1}{#2}| at the preamble to create
the combined table of contents.

\verb|\wstoc{Article Title}{Author's Name}|

\section{Preparing the Individual Contributions for Combining}

The following highlighted changes should be made in all the contributions provided by the individual contributors before including them in the master document.

\begin{verbatim}
Contribution provided by an        Modified contribution, ready to
individual contributor:            get included in the master
                                   document:

%proc1.tex                         %proc1.tex
\documentclass{ws-procs961x669}     \markboth{A. Author}{Paper title}
\begin{document}                   \wstoc{Paper title}{A. Author}
\title{PAPER TITLE}                \title{Paper title}
\author{A. AUTHOR}                 \author{A. Author}
                                   \aindx{Author, A.}
\address{Institute of ...}         \address{Institute of ...}
\begin{abstract}                   \begin{abstract}
We search for ...                  We search for ...
\end{abstract}                     \end{abstract}
\keywords{Keyword1; ...}           \keywords{Keyword1; ...}
\bodymatter                        \bodymatter
\section{Introduction}             \section{Introduction}
String theory ...                  String theory ...
\begin{thebibliography}{00}        \begin{thebibliography}{00}
\bibitem{t1} A. Sen, ...           \bibitem{t1} A. Sen, ...
\bibitem{t2} P. Horava, ...        \bibitem{t2} P. Horava, ...
...                                ...
\end{thebibliography}              \end{thebibliography}
%for BiBTeX users                  %for BiBTeX users
%\bibliographystyle{ws-pro...}     %\bibliographystyle{ws-pro...}
%\bibliography{sample}             %\bibliography{sample}
\end{document}                     \vfill
                                   \pagebreak
\end{verbatim}

\section{Author Index}

To create an ``author'' index, the following
declarations should be included in the master \TeX{}
file:

\begin{verbatim}
\makeindex{author}      % in the preamble to invoke author index
\printindex{author}{AUTHOR INDEX} % at end to print author index
\end{verbatim}

In text, the author index entries are marked with:

\verb|\index{autor}{entry}| or \verb|\aindx{entry}|

\section{Compiling the Master File in \LaTeX2e}

To complete the job, compile your file as follows:

\begin{enumerate}[(4)]
\item latex ws-procs961x669
\item latex ws-procs961x669
\item bibtex~proc2\hskip48pt{\tt\% Chapters using \btex{} database should}\\
\verb|           |\hskip45pt {\tt \% be compiled individually in `bibtex'.}
\item makeindex author\hskip25pt {\tt \% author index}
\item latex ws-procs961x669
\item latex ws-procs961x669
\end{enumerate}

\begin{thebibliography}{9}
\bibitem{lamp94}
L.~Lamport, \emph{\LaTeX, A Document Preparation System}. (Addison-Wesley,
  Reading, MA, 1994), 2nd edition.
\bibitem{lamp87} L. Lamport, \emph{Make Index: An Index Processor For LaTeX}, (1987).
\end{thebibliography}

%\end{document}


==> proc2.tex <==
%\documentclass[draft]{ws-procs961x669}
%\documentclass{ws-procs961x669}

%\begin{document}

\wstoc{For proceedings contributors: Using World Scientific's\\ WS-procs961x669 document class in \LaTeX2e}
{A. B. Author and C. D. Author}

\title{For proceedings contributors:\\ Using World Scientific's WS-procs961x669\\ document class with \LaTeX2e}

\author{A. B. Author$^*$ And C. D. Author}
\index{author}{Author, A. B.} % or \aindx{Author, A. B.}
\index{author}{Author, C. D.} % or \aindx{Author, C. D.}

\address{University Department, University Name,\\
City, State ZIP/Zone, Country\\
$^*$E-mail: ab\_author@university.com\\
www.university\_name.edu}

\author{A. N. Author}

\address{Group, Laboratory, Street,\\
City, State ZIP/Zone, Country\\
E-mail: an\_author@laboratory.com}

\begin{abstract}
This article explains how to use World Scientific's ws-procs961x669
document class written in \LaTeX2e. This article was typeset using
ws-procs961x669.cls and may be used as a template for your contribution.
\end{abstract}

\keywords{Style file; \LaTeX; Proceedings; World Scientific Publishing.}

\bodymatter

\section{Using Other Packages}\label{aba:sec1}
The class file loads the packages {\tt amsfonts, amsmath, amssymb,
chapterbib, cite, dcolumn, epsfig, rotating} and {\tt url} at
startup. Please try to limit your use of additional packages as they
often introduce incompatibilities. This problem is not specific to
the WSPC styles; it is a general \LaTeX{} problem. Check this
article to see whether the required functionality is already
provided by the WSPC class file. If you do need additional packages,
send them along with the paper. In general, you should use standard
\LaTeX{} commands as much as possible.

\section{Layout}
In order to facilitate our processing of your article, please give
easily identifiable structure to the various parts of the text by
making use of the usual \LaTeX{} commands or by using your own commands
defined in the preamble, rather than by \hbox{using} explicit layout
commands, such as \verb|\hspace, \vspace, \large, \centering|,
etc.~Also, do not redefine the page-layout parameters.~For more
information on layout and font specifications, please refer to our
\verb|Layout and| \verb|Font Specification Guide|.

\section{User Defined Macros}
User defined macros should be placed in the preamble of the article,
and not at any other place in the document. Such private
definitions, i.e. definitions made using the commands
\verb|\newcommand, \renewcommand, \newenvironment| or
\verb|\renewenvironment|, should be used with great care. Sensible,
restricted usage of private definitions is encouraged. Large macro
packages and definitions that are not used in this example article
should be avoided. Please do not change the existing environments,
commands and other standard parts of \LaTeX.

\section{Using WS-procs961x669}
You can obtain these files from the following website:\\
\url{http://www.icpress.co.uk/authors/stylefiles.shtml#conference} and \\
\url{http://www.worldscientific.com/page/authors/proceedings-stylefiles}.

\subsection{Input used to produce this paper}
\begin{verbatim}
\documentclass{ws-procs961x669}
\begin{document}
\title{For proceedings contributors: ...}
\author{A. B. Author$^*$ and C. D. Author}
\address{University Department, ...}
\author{A. N. Author}
\address{Group, Laboratory, Street, ...}
\begin{abstract}
This article explains how to...
\end{abstract}
\keywords{Style file; \LaTeX,...}
\bodymatter
\section{Using Other Packages}
The class file has...
\bibliographystyle{ws-procs961x669}
\bibliography{ws-pro-sample}
\end{document}
\end{verbatim}

\subsection{Class options}
{\tablefont
\begin{tabular}{@{}ll@{}}\\
\quad\verb|\usepackage{ws-procs961x669}| & -- Superscript$^1$ (Default style)\\
\quad\verb|\usepackage[wssquare]{ws-procs961x669}| & -- Bracketed [1]\\[6pt]
\end{tabular}\\}

The contributors are advised to consult the proceedings editor before choosing the citation style \verb|wssquare|.

\section{Sectional Units}
Sectional units are obtained in the usual way, i.e. with the \LaTeX{}
commands \verb|\section|, \verb|\subsection|, \verb|\subsubsection| and \verb|\paragraph|.

\section{Section}
This is just an example.

\subsection{Subsection}
This is just an example.

\subsubsection{Subsubsection}
This is just an example.

\paragraph{Paragraph}
This is just an example.

\section*{Unnumbered Section}
Unnumbered sections can be obtained by using \verb|\section*|.

\section{Lists of Items}
Lists are broadly classified into four major categories that can
randomly be used as desired by the author:
\begin{alphlist}[(d)]
\item Numbered list.
\item Lettered list.
\item Unnumbered list.
\item Bulleted list.
\end{alphlist}

\subsection{Numbered and lettered list}

\begin{arabiclist}[(5)]
\item The \verb|\begin{arabiclist}[]| command is used for the arabic
number list (arabic numbers appearing within parenthesis), e.g.,
(1), (2), etc.

\smallskip

\item The \verb|\begin{romanlist}[]| command is used for the roman
number list (roman numbers appearing within parenthesis), e.g., (i),
(ii), etc.

\smallskip

\item The \verb|\begin{Romanlist}[]| command is used for the cap roman
\hbox{number list} (cap roman numbers appearing within parenthesis),
e.g., (I), (II), etc.

\smallskip

\item The \verb|\begin{alphlist}[]| command is used for the alphabetic
list (alphabets appearing within parenthesis), e.g., (a), (b), etc.

\smallskip

\item The \verb|\begin{Alphlist}[]| command is used for the cap
alphabetic list (cap alphabets appearing within parenthesis),
e.g., (A), (B), etc.
\end{arabiclist}
Note: For all the above mentioned lists (with the exception of
alphabetic list), it is obligatory to enter the last entry's number
in the list within the square bracket, to enable unit alignment.

\subsection{Bulleted and unnumbered list}

\begin{enumerate}
\item[] The \verb|\begin{itemlist}| command is used for the bulleted list.

\smallskip

\item[] The \verb|\begin{unnumlist}| command is used for creating the
  unnumbered list with the turnovers hangindent by 1\,pica.
\end{enumerate}

Lists may be laid out with each item marked by a dot:
\begin{itemlist}
\item item one
\item item two
\item item three
\item item four.
\end{itemlist}

Items may also be numbered with lowercase Roman numerals:
\begin{romanlist}[(iii)]
\item item one
\item item two
    \begin{alphlist}[(c)]
    \item lists within lists can be numbered with lowercase alphabets
    \item second item
    \item item three.
    \end{alphlist}
\item item three
\item item four.
\end{romanlist}

\section{Theorems and Definitions}

\noindent{\bf Input:}

\begin{verbatim}
\begin{theorem}
We have $\# H^2 (M \supset N) < \infty$ for an inclusion ...
\end{theorem}
\end{verbatim}

\noindent{\bf Output:}

\begin{theorem}
We have $\# H^2 (M \supset N) < \infty$ for an inclusion $M \supset
N$ of factors of finite index.
\end{theorem}

\noindent{\bf Input:}

\begin{verbatim}
\begin{theorem}[Longo, 1998]
For a given $Q$-system...
\[ N = \{x \in N; T x = \gamma (x) T, T x^* = \gamma (x^*) T\}, \]
and $E_\Xi (\cdot) = T^* \gamma (\cdot) T$ gives ...
\end{theorem}
\end{verbatim}

\noindent{\bf Output:}

\begin{theorem}[Longo, 1998]
For a given $Q$-system...
\[
N = \{x \in N; T x = \gamma (x) T, T x^* = \gamma (x^*) T\},
\]
and $E_\Xi (\cdot) = T^* \gamma (\cdot) T$ gives a conditional
expectation onto $N$.
\end{theorem}

The following environments are available by default with WSPC
document styles:

\begin{center}
{\tablefont
\begin{tabular}{ll}
\toprule
Environment & Heading\\\colrule
\verb|algorithm| & Algorithm\\
\verb|answer| & Answer\\
\verb|assertion| & Assertion\\
\verb|assumption| & Assumption\\
\verb|case| & Case\\
\verb|claim| & Claim\\
\verb|comment| & Comment\\
\verb|condition| & Condition\\
\verb|conjecture| & Conjecture\\
\verb|convention| & Convention\\
\verb|corollary| & Corollary\\
\verb|criterion| & Criterion\\
\verb|definition| & Definition\\
\verb|example| & Example\\
\verb|lemma| & Lemma\\
\verb|notation| & Notation\\
\verb|note| & Note\\
\verb|observation| & Observation\\
\verb|problem| & Problem\\
\verb|proposition| & Proposition\\
\verb|question| & Question\\
\verb|remark| & Remark\\
\verb|solution| & Solution\\
\verb|step| & Step\\
\verb|summary| & Summary\\
\verb|theorem| & Theorem \\\botrule
\end{tabular}}\label{aba:theo}
\end{center}

\LaTeX{} provides \verb|\newtheorem| to create new theorem
environments. To add theorem-type environments to an article, use

\begin{verbatim}
\newtheorem{example}{Example}[section]
\let\Examplefont\upshape
\def\Exampleheadfont{\bfseries}

\begin{example}
We have $\# H^2 (M \supset N) < ...
\end{example}
\end{verbatim}

For details see the \LaTeX{} user manual.\cite{lamp94,ams04}

\subsection{Proofs}
The WSPC document styles also provide a predefined proof environment
for proofs. The proof \hbox{environment} produces the heading
`Proof' with appropriate spacing and punctuation. It also appends a
`Q.E.D.' symbol, $\square$, at the end of a proof, e.g.,

\begin{verbatim}
\begin{proof}
This is just an example.
\end{proof}
\end{verbatim}

\noindent to produce

\begin{proof}
This is just an example.
\end{proof}

The proof environment takes an argument in curly
braces, which allows you to substitute a different name for the standard
`Proof'. If you want to display, `Proof of Lemma', then write e.g.

\begin{verbatim}
\begin{proof}[Proof of Lemma]
This is just an example.
\end{proof}
\end{verbatim}

\noindent produces

\begin{proof}[Proof of Lemma]
This is just an example.
\end{proof}

\section{Programs and Algorithms}
Fragments of computer programs and descriptions of algorithms should be
prepared as if they were normal text. Use the same fonts for keywords,
variables, etc., as in the text; do not use small typeface sizes to make program
fragments and algorithms fit within the margins set by the document style.
An example with only the tabbing environment and one new definition:

\begin{verbatim}
\newcommand{\keyw}[1]{{\bf #1}}
\begin{tabbing}
\quad \=\quad \=\quad \kill
\keyw{for} each $x$ \keyw{do} \\
\> \keyw{if} extension$(p, x)$ \\
\> \> \keyw{then} $E:=E\cup\{x\}$\\
\keyw{return} $E$
\end{tabbing}
\end{verbatim}

\noindent{\bf Output:}

\newcommand{\keyw}[1]{{\bf #1}}
{\small{
\begin{tabbing}
\quad \=\quad \=\quad \kill
\keyw{for} each $x$ \keyw{do} \\
\> \keyw{if} extension$(p, x)$ \\
\> \> \keyw{then} $E:=E\cup\{x\}$\\
\keyw{return} $E$
\end{tabbing}
}}

\section{Mathematical Formulas}
\paragraph{Inline:}
For in-line formulas use \verb|\( ... \)| or \verb|$ ... $|. Avoid
built-up constructions, for example fractions and matrices, in
in-line formulas. Fractions in inline can be typed with a solidus, e.g. \verb|x+y/z=0|.

\paragraph{Display:}
For numbered display formulas, use the displaymath
environment:

\begin{verbatim}
\begin{equation}
...
\end{equation}
\end{verbatim}

And for unnumbered display formulas, use
\verb|\[ ... \]|. For numbered displayed,
one-line formulas always use the equation environment. Do not use
\verb|$$ ... $$|. For example, the input for:

\begin{equation}
\mu(n, t) = \frac{\sum\limits^\infty_{i=1}1 (d_i < t, N(d_i) = n)}
{\int\limits^t_{\sigma=0}1(N(\sigma)=n)d\sigma}.
\label{aba:eq1}
\end{equation}

\noindent is:

\begin{verbatim}
\begin{equation}
\mu(n, t) = \frac{\sum\limits^\infty_{i=1}1 (d_i < t, N(d_i) = n)}
{\int\limits^t_{\sigma=0}1 (N(\sigma)=n)d\sigma}.\label{aba:eq1}
\end{equation}
\end{verbatim}

For displayed multi-line formulas, use the \verb|align| environment. For example,

\begin{verbatim}
\begin{align}
\zeta\mapsto\hat{\zeta}&=a\zeta+b\eta\label{aba:eq2}\\
\eta\mapsto\hat{\eta}&=c\zeta+d\eta\label{aba:eq3}
\end{align}
\end{verbatim}

\noindent produces:
\begin{align}
\zeta\mapsto\hat{\zeta}&=a\zeta+b\eta\label{aba:eq2}\\
\eta\mapsto\hat{\eta}&=c\zeta+d\eta\label{aba:eq3}
\end{align}

Superscripts and subscripts that are words or abbreviations, as in
\( \sigma_{\mathrm{low}} \), should be typed as roman letters;
this is done as \verb|\( \sigma_{\mathrm{low}} \)|
instead of \( \sigma_{low} \) done with \verb|\( \sigma_{low} \)|.

For geometric functions, e.g.~exp, sin, cos, tan, etc., please use the macros
\verb|\sin, \cos, \tan|. These macros give proper spacing in mathematical formulas.

It is also possible to use the \AmS-\LaTeX{}
package,\cite{ams04} which can be obtained from the \AmS\ and various \TeX{}
archives.

\section{Floats}
\subsection{Tables}
Put tables and figures in text using the table and figure environments,
and position them near the first reference of the table or figure in
the text. Please avoid long captions in figures and tables.
\vskip12pt
\noindent{\bf Input:}

\begin{verbatim}
\begin{table}
\tbl{Comparison of acoustic for frequencies for piston-cylinder
problem.}
{\begin{tabular}{@{}cccc@{}}
\toprule
Piston mass & Analytical frequency & TRIA6-$S_1$ model & ...\\
& (Rad/s) & (Rad/s) \\\colrule
1.0\hphantom{00} & \hphantom{0}281.0 & \hphantom{0}280.81 & 0.07 \\
0.1\hphantom{00} & \hphantom{0}876.0 & \hphantom{0}875.74 & 0.03 \\
0.01\hphantom{0} & 2441.0 & 2441.0\hphantom{0} & 0.0\hphantom{0} \\
0.001 & 4130.0 & 4129.3\hphantom{0} & 0.16\\\botrule
\end{tabular}}
\begin{tabnote}
$^{\text a}$ Sample table footnote.\\
\end{tabnote}
\label{aba:tbl1}
\end{table}
\end{verbatim}

\noindent {\bf Output:}

\begin{table}
\tbl{Comparison of acoustic for frequencies for piston-cylinder problem.}
{\begin{tabular}{@{}cccc@{}}
\toprule
Piston mass & Analytical frequency & TRIA6-$S_1$ model & \% Error$^{\text a}$ \\
& (Rad/s) & (Rad/s) \\
\colrule
1.0\hphantom{00} & \hphantom{0}281.0 & \hphantom{0}280.81 & 0.07 \\
0.1\hphantom{00} & \hphantom{0}876.0 & \hphantom{0}875.74 & 0.03 \\
0.01\hphantom{0} & 2441.0 & 2441.0\hphantom{0} & 0.0\hphantom{0} \\
0.001 & 4130.0 & 4129.3\hphantom{0} & 0.16\\
\botrule
\end{tabular}
}
\begin{tabnote}
$^{\text a}$ Sample table footnote.\\
\end{tabnote}
\label{aba:tbl1}
\end{table}

\def\p{\phantom{$-$}}
\def\pc{\phantom{,}}
\def\p0{\phantom{0}}
\begin{sidewaystable}
\tbl{Positive values of $X_0$ by eliminating $Q_0$ from
Eqs.~(15) and (16) for different values of the parameters $f_0$,
$\lambda_0$ and $\alpha_0$ in various dimension.}
{\begin{tabular}{@{}ccccccccccc@{}}
\toprule\\[-6pt]
$f_0$ &$\lambda_0$ &$\alpha_0$
&\multicolumn{8}{c}{Positive roots ($X_0$)}\\[3pt]
\hline\\[-6pt]
&& &4D &5D &6D &7D &8D &10D &12D &16D\\[3.5pt]
\hline\\[-6pt]
\phantom{1}$-0.033$ &0.034 &\phantom{0}0.1\phantom{.01}
&6.75507,\p0 &4.32936,\p0 &3.15991,\p0 &2.44524,\p0
&1.92883,\p0 &0.669541, &--- &---\\[3.5pt]
&&&1.14476\pc\p0 &1.16321\pc\p0 &1.1879\pc\phantom{00}
&1.22434\pc\p0 &1.29065\pc\p0
&0.415056\pc\\[3.5pt]
\phantom{1}$-0.1$\phantom{33} &0.333 &\phantom{0}0.2\phantom{.01}
&3.15662,\p0 &1.72737,\p0 &--- &--- &--- &--- &--- &---\\[3.5pt]
&&&1.24003\pc\p0 &1.48602\pc\p0\\[3.5pt]
\phantom{1}$-0.301$ &0.302 &0.001
&2.07773,\p0 &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
&&&1.65625\pc\p0\\[3.5pt]
\phantom{1}$-0.5$\phantom{01} &0.51\phantom{2} &\phantom{0}0.001
&--- &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &0.1\phantom{02}
&\phantom{0}2\phantom{.001} &1.667,\phantom{000} &1.1946\phantom{00,}
&--- &--- &--- &--- &--- &---\\[3.5pt]
&&&0.806578\pc &0.858211\pc\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &0.1\phantom{33} &10\phantom{.001}
&0.463679\pc &0.465426\pc &0.466489\pc &0.466499\pc
&0.464947\pc &0.45438\pc\p0 &0.429651\pc &0.35278\pc\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &1\phantom{.333}
&\phantom{0}0.2\phantom{01}
&--- &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &5\phantom{.333}
&\phantom{0}5\phantom{.001}
&--- &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
$\phantom{-0}$1\phantom{.033} &0.001 &\phantom{0}2\phantom{.001}
&0.996033, &0.968869, &0.91379,\p0 &0.848544,&0.783787, &0.669541,
&0.577489, &---\\[3.5pt]
&&&0.414324\pc &0.41436\pc\p0 &0.414412\pc &0.414489\pc &0.414605\pc
&0.415056\pc &0.416214\pc\\[3.5pt]
\phantom{10}\phantom{.033} &0.001 &\phantom{0}0.2\phantom{01}
&0.316014, &0.309739, &--- &--- &--- &--- &--- &---\\[3.5pt]
&&&0.275327\pc &0.275856\pc\\[3.5pt]
\phantom{10}\phantom{.033} &0.1\phantom{33}
&\phantom{0}5\phantom{.001}
&0.089435\pc &0.089441\pc &0.089435\pc &0.089409\pc &0.08935\pc\p0
&0.089061\pc &0.088347\pc &0.084352\pc\\[3.5pt]
\phantom{10}\phantom{.033} &1\phantom{.333} &\phantom{0}3\phantom{.001}
&0.128192\pc &0.128966\pc &0.19718,\p0 &0.169063, &0.142103,
&--- &--- &---\\[3.5pt]
&&&& &0.41436\pc\p0 &0.414412\pc &0.414489\pc\\[3pt]
\Hline
\end{tabular}}\label{aba:tbl2}
\end{sidewaystable}

Very large figures and tables should be placed on a separate page
by themselves. Landscape tables and figures can be typeset with the following environments:
\begin{itemize}
\item \verb|sidewaystable| and
\item \verb|sidewaysfigure|.
\end{itemize}

\noindent {\bf Example:}

\begin{verbatim}
\begin{sidewaystable}
\tbl{Positive values of ...}
{\begin{tabular}{@{}ccccccccccc@{}}
...
\end{tabular}}\label{aba:tbl2}
\end{sidewaystable}
\end{verbatim}

By using \verb|\tbl| command in table environment, long captions will be justified to the table width while the short or single line captions are centered.
\verb|\tbl{table caption}{tabullar environment}|.

For most tables, the horizontal rules are obtained by:

\begin{tabular}{ll}
{\bf toprule} & one rule at the top\\
{\bf colrule}& one rule separating column heads from\\ & data cells\\
{\bf botrule}& one bottom rule\\
{\bf Hline} & one thick rule at the top and bottom of\\ & the tables with multiple column heads\\
\end{tabular}

\

To avoid the rules sticking out at either end
of the table, add \verb|@{}| before the first and after the last descriptors, e.g.
{@{}llll@{}}. Please avoid vertical rules in tables.
But if you think the vertical rule is a must,
you can use the standard \LaTeX{} \verb|tabular| environment.

Headings which span for more than one column should be set using
\verb|\multicolumn{#1}{#2}{#3}| where \verb|#1| is the number of
columns to be spanned, \verb|#2| is the argument for the alignment
of the column head which may be either {c} --- for center
alignment; {l} --- for left alignment; or {r} --- for right
alignment, as desired by the users. Use {c} for column heads as
this is the WS style and \verb|#3| is the heading.

For the footnotes in the table environment the command is
\verb|{\begin{tabnote}<text>\end{tabnote}}|.

Tables should have a uniform style throughout the
proceedings volume. It does not matter how you place the
inner lines of the table, but we would prefer the border lines to be
of the style as shown in our sample tables.
For the inner lines of the table, it looks better
if they are kept to a minimum.

\subsection{Figures}
The preferred graphics formats are TIF and Encapsulated
PostScript (EPS) for any type of image. Our
\TeX\ installation requires EPS, but we can easily convert TIF to EPS.
Many other formats, e.g. PICT (Macintosh), WMF (Windows) and various proprietary
formats, are not suitable. Even if we can read such files, there is no guarantee
that they will look the same on our systems as on yours.
Adjust the scaling of the figure until it is correctly positioned,
and remove the declarations of the lines and any anomalous spacing.
A figure is obtained with the following commands

\begin{verbatim}
\begin{figure}
\includegraphics[width=2in]{procs-fig1}
\caption{Figure caption.} \label{aba:fig1}
\end{figure}
\end{verbatim}

\begin{figure}[t]
\begin{center}
\includegraphics[width=2in]{procs-fig1}
\end{center}
\caption{Figure caption.}
\label{aba:fig1}
\end{figure}

Side-by-side figures are obtained with:
\begin{verbatim}
\begin{figure}[b]%
\begin{center}
 \parbox{2.1in}{\includegraphics[width=2in]{procs-fig2a}}
 \figsubcap{a}}
 \hspace*{4pt}
 \parbox{2.1in}{\includegraphics[width=2in]{procs-fig2b}}
 \figsubcap{b}}
 \caption{Here are two figures side-by-side.
 (a) Figure caption for figure 2a. (b) Figure caption for figure 2b.}
\label{fig1.2}
\end{center}
\end{figure}
\end{verbatim}
\def\figsubcap#1{\par\noindent\centering\footnotesize(#1)}
\begin{figure}[b]%
\begin{center}
  \parbox{2.1in}{\includegraphics[width=2in]{procs-fig2a}\figsubcap{a}}
  \hspace*{4pt}
  \parbox{2.1in}{\includegraphics[width=2in]{procs-fig2b}\figsubcap{b}}
  \caption{Here are two figures side-by-side. (a) Figure caption for figure 2a. (b) Figure caption for figure 2b.}%
  \label{fig1.2}
\end{center}
\end{figure}

Figures Fig.~\ref{fig1.2}(a) and \fref{fig1.2}(b) are
referred with \verb|Fig.~\ref{fig1.2}(a)| and
\verb|\fref{fig1.2}(b)| commands.

\section{Cross-references}
Use \verb|\label| and \verb|\ref| for cross-references to
equations, figures, tables, sections, subsections, etc., instead
of plain numbers. Every numbered part to which one wants to refer,
should be labeled with the instruction \verb|\label|.
For example:
\begin{verbatim}
\begin{equation}
\mu(n, t) = \frac{\sum\limits^\infty_{i=1}1 (d_i < t, N(d_i) = n)}
{\int\limits^t_{\sigma=0}1 (N(\sigma)=n)d\sigma}.
\label{aba:eq1}
\end{equation}
\end{verbatim}
With the instruction \verb|\ref| one can refer to a numbered part
that has been labeled:
\begin{verbatim}
..., see also Eq. (\ref{aba:eq1})
\end{verbatim}

The \verb|\label| instruction should be typed
\begin{itemize}
\item immediately after (or one line below), but not inside the argument of
a number-generating instruction such as \verb|\section| or \verb|\caption|, e.g.:
\verb|\caption{ ... caption ... }\label{aba:fig1}|.
\item roughly in the position where the number appears, in environments
such as an equation,
\item labels should be unique, e.g., Eq. (\ref{aba:eq1}) can be labeled as
\verb|\label{aba:eq1}|, where `{\tt aba}' is author's initial and
`{\tt eq1}' the equation number.
\end{itemize}

\begin{center}{\tablefont
Some useful shortcut commands.\\[3pt]
\begin{tabular}{lll}
\toprule
Shortcut & Equivalent & Output \\
command & \TeX\ command\\\colrule
\multicolumn{3}{@{}l}{In the middle of a sentence:}\\
\verb|\eref{aba:eq1}|  & Eq.~(\verb|\ref{aba:eq1}|) & \eref{aba:eq1}\\
\verb|\sref{aba:sec1}| & Sec.~\verb|\ref{aba:sec1}| & \sref{aba:sec1}\\
\verb|\fref{aba:fig1}| & Fig.~\verb|\ref{aba:fig1}|  & \fref{aba:fig1}\\
\verb|\tref{aba:tbl1}| & Table~\verb|\ref{aba:tbl1}|  & \tref{aba:tbl1}\\[3pt]
\multicolumn{2}{@{}l}{At the starting of a sentence:}\\
\verb|\Eref{aba:eq1}|  & Equation (\verb|\ref{aba:eq1}|) & \Eref{aba:eq1}\\
\verb|\Sref{aba:sec1}| & Section~\verb|\ref{aba:sec1}| & \Sref{aba:sec1}\\
\verb|\Fref{aba:fig1}| & Figure~\verb|\ref{aba:fig1}| & \Fref{aba:fig1}\\
\verb|\Tref{aba:tbl1}| & Table~\verb|\ref{aba:tbl1}| & \Tref{aba:tbl1}\\\botrule
\end{tabular}}
\end{center}

\section{Citations}
We have used \verb|\bibitem| to produce the bibliography. Citations in the
text use the labels defined in the bibitem declaration, e.g.,
the first paper by Jarlskog\cite{jarl88} is cited using the command
\verb|\cite{jarl88}|. Bibitem labels should be unique.

For multiple citations, do not use \verb|\cite{1}|, \verb|\cite{2}|, but use
\verb|\cite{1,2}| instead.

When the reference forms part of the sentence, it should not
be typed in superscripts, e.g.: ``One can show from
Ref.~\citenum{jarl88} that $\ldots$'', ``See
Refs.~\citenum{lamp94} and \citenum{ams04} for more details.''
This is done using the \LaTeX{} command: ``\verb|Ref.~\citenum{name}|''.

\section{Footnotes}
Footnotes are denoted by a Roman letter superscript in the text. Footnotes can be used as

\

\noindent {\bf Input:}
\begin{verbatim}
... total.\footnote{Sample footnote text.}
\end{verbatim}

\noindent {\bf Output:}

\noindent ... in total.\footnote{Sample footnote text.}

\section{Acknowledgments and Appendices}
Acknowledgments to funding bodies etc.~may be placed in a separate
section at the end of the text, before the Appendices. This should not
be numbered, so use \verb|\section*{Acknowledgments}|.

It is preferable to have no appendices in a short article, but if
it is necessary, then simply use as

\begin{verbatim}
\appendix{About the Appendix}
Appendices should be...
\begin{equation}
\mu(n, t) = \frac{\sum^\infty_{i=1} 1(d_i < t, N(d_i) = n)}
{\int^t_{\sigma=0} 1(N(\sigma) = n)d\sigma}. \label{aba:aeq1}
\end{equation}
\subappendix{Appendix Sectional Units}
Sectional units are...
\end{verbatim}

\section{References}
References are to be listed in the order cited in the text in Arabic
numerals. \btex users, please use our bibliography style file
\verb|ws-procs961x669.bst| for references.

Non \btex\ users can list down their references in the following pattern.

\begin{verbatim}
\begin{thebibliography}{9}
\bibitem{lam94} L.~Lamport, {\it\LaTeX, A Document Preparation
    System}, 2nd edn. (Addison-Wesley, Reading, 1994).
\bibitem{ams04} \AmS, {\it \AmS-\LaTeX{} Version 2 User's
    Guide} (American Mathematical Society, Providence, 2004),
    \url{http://www.ams.org/tex/amslatex.html}.
\bibitem{jarl88} C.~Jarlskog, {\it CP {V}iolation}
    (World Scientific, Singapore, 1988).
\bibitem{best03} B.~W. Bestbury, $R$-matrices and the magic
    square, {\it J. Phys. A} {\bf 36}, 1947 (2003).
\bibitem{jame02} J.~M. Landsberg and L.~Manivel, Triality,
    exceptional Lie algebras and Deligne dimension formulas,
    {\it Adv. Math.} {\bf 171}, 59 (2002),
    \url{http://www.url.com/triality.html}.
\end{thebibliography}
\end{verbatim}

\section{{\btex}ing}
If you use the \btex\ program to maintain your bibliography, you do
not use the \verb|thebibliography| environment. Instead, you should
include the lines

\begin{verbatim}
\bibliographystyle{ws-procs961x669}
\bibliography{ws-pro-sample}
\end{verbatim}

\noindent where \verb|ws-procs961x669| refers to a file \verb|ws-procs961x669.bst|,
which defines how your references will look.
The argument to \verb|\bibliography| refers to the file
\verb|ws-pro-sample.bib|, which should contain your database in
\btex\ format. Only the entries referred to via \verb|\cite| will be
listed in the bibliography.

Sample output using \verb|ws-procs961x669| bibliography style file:

\begin{center}
\tablefont
\begin{tabular}{@{}ll@{}}\toprule
\multicolumn{1}{c}{\btex}\\
\multicolumn{1}{c}{database}  & \multicolumn{1}{c}{Sample citation}\\
\multicolumn{1}{c}{entry type}\\\colrule

article & ... text.\cite{best03,pier02,jame02}\\

proceedings & ... text.\cite{weis94}\\

inproceedings & ... text.\cite{gupt97}\\

book & ... text.\cite{jarl88,rich60}\\

edition & ... text.\cite{chur90}\\

editor & ... text.\cite{benh93}\\

series & ... text.\cite{bake72}\\

tech report & See Refs.~\citenum{hobb92} and \citenum{bria84} for more details\\

unpublished & ... text.\cite{hear94}\\

phd thesis & ... text.\cite{brow88}\\

masters thesis & ... text.\cite{lodh74}\\

incollection & ... text.\cite{dani73}\\

misc & ... text.\cite{davi93}\\
\botrule
\end{tabular}
\end{center}

\eject

\appendix{About the Appendix}
Appendices should be used only when absolutely necessary. They
should come before the References.

\subappendix{Appendix Sectional Units}
Where two or more appendices are used, number them alphabetically.
Sectional units are obtained with the \LaTeX{} commands:

\begin{itemlist}
\item \verb|\appendix|
\item \verb|\subappendix|.
\end{itemlist}

Unnumbered appendix sections can be obtained using \verb|\section*|.

\begin{table}
\tbl{Macros available for use in text.}
{\begin{tabular}{@{}ll@{}}
\toprule
Macro name&Purpose\\
\colrule
{\tt$\backslash$title}\{{\tt\#1}\} & Article title\\
{\tt$\backslash$author}\{{\tt\#1}\} & List of all authors\\
{\tt$\backslash$address}\{{\tt\#1}\} & Address of author\\
{\tt$\backslash$begin}\{{\tt{abstract}}\}...{\tt$\backslash$end}\{{\tt{abstract}}\} & Abstract\\
{\tt$\backslash$keywords}\{{\tt\#1}\} & Keywords\\
{\tt$\backslash$bodymatter} & Start body text\\
{\tt$\backslash$section}\{{\tt\#1}\} & Section heading\\
{\tt$\backslash$subsection}\{{\tt\#1}\} & Subsection heading\\
{\tt$\backslash$subsubsection}\{{\tt\#1}\} & Subsubsection heading\\
{\tt$\backslash$section*}\{{\tt\#1}\} & Unnumbered Section head\\
{\tt$\backslash$begin}\{{\tt{itemlist}}\} & Start bulleted lists\\
{\tt$\backslash$end}\{{\tt{itemlist}}\} & End bulleted lists\\
{\tt$\backslash$begin}\{{\tt{arabiclist}}\} & Start arabic lists (1, 2, 3...)\\
{\tt$\backslash$end}\{{\tt{arabiclist}}\} & End arabic lists\\
{\tt$\backslash$begin}\{{\tt{romanlist}}\} & Start roman lists (i, ii, iii...)\\
{\tt$\backslash$end}\{{\tt{romanlist}}\} & End roman lists\\
{\tt$\backslash$begin}\{{\tt{Romanlist}}\} & Start roman lists (I, II, III...)\\
{\tt$\backslash$end}\{{\tt{Romanlist}}\} & End roman lists\\
{\tt$\backslash$begin}\{{\tt{alphlist}}\} & Start alpha lists (a, b, c...)\\
{\tt$\backslash$end}\{{\tt{alphlist}}\} & End alpha lists\\
{\tt$\backslash$begin}\{{\tt{Alphlist}}\} & Start alpha lists (A, B, C...)\\
{\tt$\backslash$end}\{{\tt{Alphlist}}\} & End alpha lists\\
{\tt$\backslash$begin}\{{\tt{proof}}\} & Start of Proof\\
{\tt$\backslash$end}\{{\tt{proof}}\} & End of Proof\\
{\tt$\backslash$begin}\{{\tt{theorem}}\} & Start of Theorem\\
{\tt$\backslash$end}\{{\tt{theorem}}\} & End of Theorem (See Page \pageref{aba:theo} for more details)\\
{\tt$\backslash$appendix}\{{\tt\#1}\} & Appendix Section heading\\
{\tt$\backslash$subappendix}\{{\tt\#1}\} & Appendix Subsection heading\\
{\tt$\backslash$begin}\{{\tt{thebibliography}}\}\{{\tt\#1}\} & Start of numbered reference list\\
{\tt$\backslash$bibitem}\{{\tt\#1}\} & Reference item in numbered style\\
{\tt$\backslash$end}\{{\tt{thebibliography}}\} & End of numbered reference list\\
{\tt$\backslash$bibliographystyle}\{{\tt\#1}\} & To include \btex{} style file\\
{\tt$\backslash$bibliography}\{{\tt\#1}\} & To include \btex{} database\\
{\tt$\backslash$blankpage} & blank page with no running heads\\  \botrule
\end{tabular}}
\end{table}

\begin{table}
\tbl{Macros available for tables/figures.}
{\begin{tabular}{@{}ll@{}}
\toprule
Environment name&Purpose\\
\colrule
{\tt figure} & Figures\\
{\tt sidewaysfigure} & Landscape figures\\
{\tt table} & Tables\\
{\tt sidewaystable} & Landscape tables\\ \colrule
Horizontal rules & Purpose\\ \colrule
{\tt $\backslash$toprule} & One rule at the top\\
{\tt $\backslash$colrule} & One rule separating column heads from\\ & data cells\\
{\tt $\backslash$botrule} & One bottom rule\\
{\tt $\backslash$Hline} & One thick rule at the top and bottom of\\
& the tables with multiple column heads\\ \botrule
\end{tabular}}
\end{table}

Number displayed equations
occurring in the Appendix in this way, e.g.~(\ref{aba:aeq1}), (\ref{aba:aeq2}),
etc.

\noindent\begin{align}
\zeta\mapsto\hat{\zeta}&=a\zeta+b\eta\label{aba:aeq1}\\
\eta\mapsto\hat{\eta}&=c\zeta+d\eta\label{aba:aeq2}
\end{align}

\appendix{Sample Appendix}
Sample text...
\begin{equation}
\mu(n, t) = \frac{\sum^\infty_{i=1} 1(d_i < t, N(d_i) = n)}
{\int^t_{\sigma=0} 1(N(\sigma) = n)d\sigma}. \label{aba:aeq3}
\end{equation}

\bibliographystyle{ws-procs961x669}
\bibliography{ws-pro-sample}

%\end{document}

